Introducing Geometry in Active Learning for Image Segmentation

We propose an Active Learning approach to training a segmentation classifier that exploits geometric priors to streamline the annotation process in 3D image volumes. To this end, we use these priors not only to select voxels most in need of annotation but to guarantee that they lie on 2D planar patch, which makes it much easier to annotate than if they were randomly distributed in the volume. A simplified version of this approach is effective in natural 2D images. We evaluated our approach on Electron Microscopy and Magnetic Resonance image volumes, as well as on natural images. Comparing our approach against several accepted baselines demonstrates a marked performance increase.

==> fig/05-2planes.tex <==
\begin{figure}[t]
\begin{center}
   \includegraphics[width=1\linewidth]{2planesnotation.pdf}
\end{center}
   \caption{Two  planes  $P_{\min}$ and  $P_{\max}$  defined  by pairs  of  angles
     ($\phi_{\min}$, $\gamma_{\min}$) and ($\phi_{\max}$, $\gamma_{\max}$). Each
     plane  has norm  $\vec{n}_{\min}$  and $\vec{n}_{\max}$.  Green points  are
     included as  lying between  planes, their  doc product  with both  norms is
     positive or negative. Black points are not included.}
   \label{fig:05-2planes}
\end{figure}


==> fig/05-pseudocode.tex <==
\begin{algorithm}[h] 
\caption{Search for an optimal plane}
\begin{algorithmic} \label{alg:overview}
\REQUIRE set of all supervoxels approximation $\hat{S} = \{ (w_j), \kappa \}$, \\
uncertainty values $U$ where $U(\hat{s}_j)$ is the value for supervoxel $\hat{s}_i$, \\
set of $t$ top supervoxels with the highest uncertainty -- $S^t$,  \\
$r$ \\
\STATE compute $\alpha_{\min}$ \COMMENT{Eq.~\ref{}} 
\FOR {$\hat{s}_i \in \hat{S}^t$}
	\STATE find $\hat{S}_i^r$ \\ 
	\STATE start list of regions $L={[l]}$ with $l= {[\phi_{\min}; \phi_{\max}; \gamma_{\min}; \gamma_{\max}; v]}$, where $\phi_{\min} = 0$, $\phi_{\max} = \pi$, $\gamma_{\min} = 0$, $\gamma_{\max} = \pi$, $v = \sum\limits_{\hat{s}_k \in \hat{S}^{r^p}} U(\hat{s}_k)$
	\STATE $\alpha_{\max} \gets \phi_{\max}-\phi_{\min}$
	\WHILE {$\alpha_{\max}>\alpha_{\min}$}
		\STATE split last region in $L$ into 2: \\ 
		\begin{equation*}
		l_1 = [\phi_{\min}; \frac{\phi_{\min}+\phi_{\max}}{2}; \gamma_{\min}; \frac{\gamma_{\min}+\gamma_{\max}}{2}; v_1 ]
		\end{equation*} 
		and 
		\begin{equation*}
		l_2 = [\frac{\phi_{\min}+\phi_{\max}}{2}; \phi_{\max}; \frac{\gamma_{\min}+\gamma_{\max}}{2}; \gamma_{\max}; v_2 ]
		\end{equation*}
		\FOR {$l_j = [l_1; l_2]$}
			\STATE $p_{\min} = (l_j(1),l_j(3))$ 
			\STATE $p_{\max} = (l_j(2),l_j(4))$
			\STATE find $\vec{n}_{\min}, \vec{n}_{\max}$
			\STATE $d=\vec{n}_{\min} \vec{n}_{\max}$
			\IF {$p > 0$}
				\STATE change orientation of one one of them: \\ $\vec{n}_{\min} \gets -\vec{n}_{\min}$ 
			\ENDIF
			\STATE select the supervoxels between these planes $C_i^r(p_{\min},p_{\max})$ Eq.~ref{}
			\STATE $v_j = \sum\limits_{\hat{s}_k \in C_i^r(p_{\min}, p_{\max})} U(\hat{s}_k)$
		\ENDFOR
		\STATE insert $l_1,l_2$ into $L$ so that regions are sorted by $v$ in ascending order
		\STATE $\alpha_{\max} = L(end,2)-L(end,1)$
	\ENDWHILE
	\STATE the best plane going through supervoxels $s_i$ has value $v(s_i)=L(end,5)$
\ENDFOR
\STATE select the plane with highest value $s^* = \underset{s_i \in S^t}{\arg\max} v(s_i)$
\RETURN voxel $s^*$ with its corresponding $C_i^r(p_{\min}, p_{\max})$
\end{algorithmic}
\end{algorithm}

==> fig/06-mri-r.tex <==
\begin{figure}[h]
\begin{center}
   \includegraphics[width=0.8\linewidth]{mri-r.pdf}
\end{center}
   \caption{Geometry plane selection with different radius of patch}
   \label{fig:06-mri-r}
\end{figure}

==> fig/framework.tex <==
\begin{figure}[t]
\begin{center}
%\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   \includegraphics[width=0.8\linewidth]{activelearning.eps}
\end{center}
   \caption{Active Learning pipeline: we start with a small labelled dataset $X_L$, $Y_L$, train a model with parameters $\theta$} and select datapoints for querying a user based on the predictions on unlabelled dataset $X_U$.
\label{fig:active}
\end{figure}


==> fig/intro.tex <==
\begin{figure}
\centering
\begin{tabular}{@{\hspace{1cm}}c@{\hspace{2cm}}c@{\hspace{1cm}}c@{\hspace{2pt}}}

\multicolumn{3}{l}{\includegraphics[width=1\linewidth]{intro_v6.pdf}}
%
\comment{
\includegraphics[width=0.33\linewidth]{road_7_and_gt.pdf}&
{%
\setlength{\fboxsep}{0pt}%
\setlength{\fboxrule}{1pt}%
\fboxrule=0.05pt%
  \fbox{%
\includegraphics[width=0.33\linewidth]{road_7_tubularity.pdf}
}}&%
{%
\setlength{\fboxsep}{0pt}%
\setlength{\fboxrule}{1pt}%
\fboxrule=0.05pt%
  \fbox{%
\includegraphics[width=0.33\linewidth]{road_7_scale_space_tubularity_NN_iters_1.pdf}%
}}\\%

}\\
%\includegraphics[width=0.15\linewidth]{d_func_crop2}&
%\includegraphics[width=0.15\linewidth]{bf_crop_learn}&
%\includegraphics[width=0.15\linewidth]{bf_crop_nms}\\
%\footnotesize  Raw  & \footnotesize Ground Truth & \footnotesize
%Distance& \footnotesize  $d$ function& \footnotesize  Learned  \\[-1.0ex]
%\footnotesize Image & \footnotesize Centerline   & \footnotesize  Transform & \footnotesize & \footnotesize Function
\footnotesize  (a) Image & \footnotesize (b) \cite{Sironi15b} & \footnotesize (c) Ours% & \footnotesize (d)  &  \footnotesize (e)  & \footnotesize (f) \\[-1.0ex]
%\footnotesize  Image& \footnotesize Centerline   & \footnotesize  Distance & \footnotesize Function & \footnotesize Function  &\footnotesize NMS \\[-1.0ex]
%\footnotesize Image & \footnotesize  $C$  & \footnotesize  $\mathcal{D}_{C}$ & \footnotesize $d$ & \footnotesize $\varphi$ &\footnotesize Image
\end{tabular}
\vspace{0.1em}
\caption{Pixel-wise classifiers reach state-of-the-art performance in
  several computer vision tasks. However, the response of such methods
  does not take into account the very particular structure and the
  spatial relation present in the ground truth images. (a) An aerial
  road image. For this problem the ground truth is composed by a continuous 1-D curve. 
 (b) Output of a state-of-the-art method~\cite{Sironi15b}. Since this
  method is based on pixel-wise regression, its output presents
  discontinuities on the centerlines and isolated responses on the
  background. (c) The output of our method is obtained by
  projecting the patches of the score image of (b) into the closest train
  ground truth patches. In this way the structure of the ground truth patches is transferred to the score image, resulting in a provably correct global spatial structure. %(d) Enlarged images of the details in the red squares in (a - top), (b - middle) and (c - bottom).
}
%\vspace{-3mm}
\label{fig:intro}
\end{figure}


==> fig/sup1.tex <==
\begin{figure}[h]
\begin{center}
   \includegraphics[width=1\linewidth]{sup1.pdf}
\end{center}
   \caption{Supervoxel approximation. Each supervoxel can be considered as a sphere of radius $\kappa$ and center $w_j$. We are interested in the neighbourhood of supervoxel $s_i$ defined by a sphere of radius $r$.}
   \label{fig:sup1}
\end{figure}


==> fig/sup2.tex <==
\begin{figure}[h]
\begin{center}
   \includegraphics[width=0.9\linewidth]{coordSys.pdf}
\end{center}
   \caption{Coordinate system for planes. We are looking for a circular patch that is defined as the intersection of a plane with a sphere. Plane $p_i$ (yellow) is defined by two angles, $\phi$ -- the intersection between plane $p$ and plane $X s_i Y$ (blue) and $\gamma$ -- the intersection between plane $p$ and plane $Y s_i Z$ (red). Best seen in colour.}
   \label{fig:sup2}
\end{figure}

==> fig/sup3.tex <==
\begin{figure}[h]
\begin{center}
   \includegraphics[width=1\linewidth]{sup3.pdf}
\end{center}
\caption{Sector splitting procedure. $U(p_0)<U([p_{\min},p_{\max}])$. We split the sector $[p_{\min},p_{\max}]$ into $[p_{\min}, p_0]$ and $[p_0, p_{\max}]$ and evaluate their uncertainty values. Among all available sectors we select a sector with the highest value to be split next. Best seen in colour.}
   \label{fig:sup3}
\end{figure}


==> fig/sup4.tex <==
\begin{figure}[h]
\begin{center}
   \includegraphics[width=0.9\linewidth]{sup4.pdf}
\end{center}
   \caption{Sector. Sector is the area between $p_{\min}$ and $p_{\max}$. Points correspond to supervoxel centres. Green points are included into sector $[p_{\min}, p_{\max}]$ and black points are not included. $\vec{n}_{\min}$ and $\vec{n}_{\max}$ are normals to planes $p_{\min}$ and $p_{\max}$. Best seen in colour.}
   \label{fig:sup4}

\end{figure}


==> fig/sup5.tex <==
\begin{figure}[h]
\begin{center}
   \includegraphics[width=0.9\linewidth]{sup5.pdf}
\end{center}
   \caption{Minimal angle of interest. The search procedure is terminated when the angle of a sector becomes less than the angle allowing to fit a single supervoxel at the end of the sector.}
   \label{fig:sup5}
\end{figure}

